Steering Masked Discrete Diffusion Models via Discrete Denoising Posterior Prediction

Generative modeling of discrete data underlies important applications spanning text-based agents like ChatGPT to the design of the very building blocks of life in protein sequences. However, application domains need to exert control over the generated data by steering the generative process - typically via RLHF - to satisfy a specified property, reward, or affinity metric. In this paper, we study the problem of steering Masked Diffusion Models (MDMs), a recent class of discrete diffusion models that offer a compelling alternative to traditional autoregressive models. We introduce Discrete Denoising Posterior Prediction (DDPP), a novel framework that casts the task of steering pre-trained MDMs as a problem of probabilistic inference by learning to sample from a target Bayesian posterior. Our DDPP framework leads to a family of three novel objectives that are all simulation-free, and thus scalable while applying to general non-differentiable reward functions. Empirically, we instantiate DDPP by steering MDMs to perform class-conditional pixel-level image modeling, RLHF-based alignment of MDMs using text-based rewards, and finetuning protein language models to generate more diverse secondary structures and shorter proteins. We substantiate our designs via wet-lab validation, where we observe transient expression of reward-optimized protein sequences.

==> iclr_space_hax.tex <==
%\def\setstretch#1{\renewcommand{\baselinestretch}{#1}}
%\setstretch{0.99}
\makeatletter
\providecommand{\section}{}
\renewcommand{\section}{%
  \@startsection{section}{1}{\z@}%
                {-1.0ex \@plus -0.5ex \@minus -0.2ex}%
                { 1.0ex \@plus  0.3ex \@minus  0.2ex}%
                {\large\sc\raggedright}%
}
\providecommand{\subsection}{}
%\renewcommand{\subsection}{%
%  \@startsection{subsection}{2}{\z@}%
%                {-0.75ex \@plus -0.5ex \@minus -0.2ex}%
%                { 0.75ex \@plus  0.2ex}%
%                {\normalsize\sc\raggedright}%
%}
\providecommand{\subsubsection}{}
\renewcommand{\subsubsection}{%
  \@startsection{subsubsection}{3}{\z@}%
                {-0.5ex \@plus -0.5ex \@minus -0.2ex}%
                { 0.5ex \@plus  0.2ex}%
                {\normalsize\sc\raggedright}%
}
\providecommand{\paragraph}{}
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}{\z@}%
                {0.3ex \@plus 0.2ex \@minus 0.2ex}%
                {-1em}%
                {\normalsize\bf}%
}
  % \linespread{0.99}
  \setlength{\textfloatsep}{5mm}

\parskip=4pt
\setlength{\abovedisplayskip}{1mm}
\setlength{\belowdisplayskip}{1mm}
\setlength{\abovedisplayshortskip}{1mm}
\setlength{\belowdisplayshortskip}{1mm}
\makeatother

==> old_method.tex <==
\section{Posterior Sampling via \name}
\label{sec:finetuning}
\looseness=-1
Given access to a pretrained masked discrete diffusion model $p_0^{\text{pre}}(\bx_0)$ we wish to sample from the reward-induced Bayesian posterior distribution $\pi_0(\bx_0)$ $\propto p_0^{\text{pre}}(\bx_0) R(\bx_0)$. We solve this sampling problem by first defining a time-dependent masking forward process that progressively adds noise to $\pi_0$ yielding the noisy reward-induced posterior $\pi_t(\bx_t) = \sum_{\bx_0} \pi_t(\bx_t | \bx_0) \pi_0(\bx_0)$, where we set $\pi_t(\bx_t | \bx_0) = p_t(\bx_t | \bx_0)$ as it is the same masking process for the pretrained MDM. 
Unfortunately, computing $\pi_t(\bx_t)$ is intractable due to the summation over $\bx_0$ and also because $p_0^{\text{pre}}(\bx_0)$ being an MDM does not easily provide an exact likelihood. Despite the intractibility of $\pi_t(\bx_t)$ we seek to approximate the reverse process $\pi_t(\bx_{t-1} | \bx_{t})$ tied to the masking forward process by using another parametrized model $q_{t, \theta}(\bx_0 | \bx_t) = \text{Cat}(\bx_0; \mu_{\theta}(\bx_t, t))$ which we take be an MDM with parameters $\theta$.


\looseness=-1
\xhdr{Denoising reward-induced posterior $\pi_t(\bx_0 | \bx_t)$}
To approximate the reverse process using an MDM we require matching the denoising reward-induced posterior $\pi_t(\bx_0 | \bx_t)$ across all masking levels---i.e. through time $t\in [0,1]$. Assisted in this endeavor, we recall the fact that since $p_0^{\text{pre}}(\bx_0)$ is also an MDM we have direct access to the pre-trained model's denoising posterior over endpoints conditioned on a partially masked sample $\bx_t$, i.e. the model parametrization is $p^{\text{pre}}_t(\bx_0 | \bx_t) = \text{Cat}(\bx_0; \mu(\bx_t, t))$. Leveraging this fact enables us to express the denoising reward-induced target posterior using a simple expression that directly uses pretrained model's denoising posterior $p^{\text{pre}}_t(\bx_0 | \bx_t)$ as follows:
\begin{align}
    \pi_{t}(\bx_0 | \bx_t) &= \frac{p_t(\bx_t | \bx_0)\pi_0(\bx_0)}{ \sum_{\bx_0'}p_t(\bx_t \mid \bx_0')  \pi_0(\bx_0')} \nonumber\\
   % &= \frac{p_t(x_t \mid x_0)p^{\text{pre}}(x_0) R(x_0)}{ \sum_{x_0'}p_t(x_t \mid x_0')  p^{\text{pre}}(x_0') R(x_0')} \\
     &= \frac{p_t(\bx_t)}{p_t(\bx_t)} \cdot \frac{p_t(\bx_t | \bx_0)p^{\text{pre}}(\bx_0) R(\bx_0) }{\sum_{\bx_0'}p_t(\bx_t | \bx_0')  p^{\text{pre}}(\bx_0') R(\bx_0') } \nonumber \\
    %&= \frac{p^{\text{pre}}_t(x_0 \mid x_t) R(x_0) p_t(x_t)}{\sum_{x_0'}p_t(x_t \mid x_0')  p^{\text{pre}}(x_0') R(x_0')} \nonumber \\
    &= \frac{p^{\text{pre}}_t(\bx_0 | \bx_t) R(\bx_0)}{\gZ_{\pi_t}(\bx_t)}.
    \label{eqn:fine_tune_posterior}
\end{align}
\looseness=-1
The expression in \eqref{eqn:fine_tune_posterior} follows from a simple application of Bayes rule and defines the normalization constant $\gZ_{\pi_t}(\bx_t) = \pi_t(\bx_t) / p_t(\bx_t)$ as the ratio between the noisy marginals of the reward-induced posterior $\pi_t(\bx_t)$ and $p_t(\bx_t)$. We make the observation that the form of $\pi_t(\bx_0 | \bx_t)$ does not require computing the intractable likelihood of a sample under the pre-trained model $p_0^{\text{pre}}(\bx_0)$, but instead makes use of the pre-trained model's posterior $p^{\text{pre}}_t(\bx_0 | \bx_t)$ which is simple to compute for an MDM. If the approximation $q_{t, \theta}$ matches the denoising reward-induced posterior we can simulate the reverse process of  $q_{t, \theta}$ to draw samples that approximately follow $\pi_0(\bx_0)$. 
Consequently, we term $q_{t, \theta}(\bx_0 | \bx_t)$ the \emph{finetuned MDM} which solves the probabilistic inference task of sampling from $\pi_0(\bx_0)$. 

\looseness=-1
In contrast to learning MDMs from a known dataset---as done when minimizing the forward KL divergence---the target denoising posterior ~\eqref{eqn:fine_tune_posterior} requires the computation of the intractable log partition function $\log \gZ_{\pi_t}(\bx_t)$ evaluated at $\bx_t$.
This observation motivates the design of three concrete learning objectives for posterior matching, which as a collection we term the \name framework. Specifically, finetuning $q_{t, \theta}$ under a \nameshort framework can be done in the following algorithms: 1.) \nameshort-IS which uses a Monte Carlo based importance sampling estimate to approximate the normalizing constant of the denoising Bayesian posterior, 2.) \nameshort-LB that constructs a lower bound to \nameshort-IS that is cheaper to evaluate by parameterizing the normalizing constant, and 3.) \nameshort-KL which uses a powerful low variance discrete gradient estimator to bypass computing the normalizing constant at the cost of requiring a differentiable reward. 
An algorithmic description of \nameshort is provided in Algorithms~\ref{alg:ft_post_pred} and ~\ref{alg:ft_reverse_KL}.




\subsection{Finetuning via Posterior Prediction}
\label{sec:posterior_prediction}
\looseness=-1
The choice of parameterizing $q_{t, \theta}(\bx_0 | \bx_t)$ as another MDM offers a prescriptive strategy for sampling from the desired target $\pi_0$ by learning to match the denoising reward-induced posterior $\pi_t(\bx_0 | \bx_t)$ at all times $t \in [0,1]$. In particular, we propose a posterior predictive objective in the discrete setting that learns $q_{t, \theta}$ in a numerically stable manner by matching the log ratio between the fine-tuning posterior of the model being learned and the denoising reward-induced posterior associated with the target:
\begin{align}
    \mathcal{L}^{\text{PP}} &= \mathbb{E}_{t, \bx_0, \bx_t} \left[ \left|\left| \log q_{t,\theta} (\bx_0 | \bx_t) - \log \pi_t(\bx_0 | \bx_t)\right| \right|^2_2\right] \nonumber \\
    \mathcal{L}^{\text{PP}} &=  \mathbb{E}_{t, \bx_0, \bx_t} \left[ \left|\left| \log q_{t,\theta} (\bx_0 | \bx_t) - \underbrace{\log p^{\text{pre}}_t(\bx_0 | \bx_t) -\log R(\bx_0) + \log \gZ_{\pi_t}(\bx_t)}_{\log \pi_t(\bx_0 | \bx_t)} \right| \right|^2_2\right].
    \label{eqn:finetune_loss}
\end{align}
\looseness=-1
Here the expectation is taken uniformly over time $t \sim \gU[0,1]$, a clean sample from some known distribution $\bx_0 \sim r(\bx_0)$, and a partially masked sample $\bx_t \sim p(\bx_t | \bx_0)$.
Inspecting the posterior predictive objective in \eqref{eqn:fine_tune_posterior} we remark that it is a simulation-free stochastic regression objective which does not require a differentiable reward as the loss computes $R(\bx_0)$ and not a gradient of the reward. Consequently, this makes the posterior predictive objective both a scalable and efficient objective for fine-tuning large pre-trained MDMs as long the reward model is easy to evaluate. Moreover, the posterior predictive objective is also an \emph{off-policy} objective as it can be evaluated using any partially masked samples $\bx_t \sim p(\bx_t | \bx_0)$. Practically, this means that fine-tuning can be performed using a replay buffer of samples from a biased dataset, e.g. the original training set for $p_0^{\text{pre}}$, or even partially masked sequences that arrive from a different model altogether. Despite its simple form the posterior predictive objective
requires the computation of the log partition function of a partially masked sequence $\log \gZ_{\pi_t}$ which does not have a closed-form expression and must be estimated.

==> old_tables.tex <==
\begin{table}[ht]
\centering
\caption{High $\beta$-sheet-content protein generation. }
\begin{tabular}{lllll}
\toprule
 & $\beta$-sheet \% & pLDDT & pTM & $\log R(x_0)$ \\
\midrule
Base Model & 0.111 $\pm$ 0.121 & 0.724 $\pm$ 0.144 & 0.584 $\pm$ 0.226 & 2.070 $\pm$ 0.749 \\
Best-of-10 & 0.280 $\pm$ 0.093 & 0.812 $\pm$ 0.033 & 0.786 $\pm$ 0.035 & 3.212 $\pm$ 0.371 \\
RTB & 0.319 $\pm$ 0.218 & 0.806 $\pm$ 0.059 & 0.767 $\pm$ 0.101 & 3.386 $\pm$ 1.061 \\
SVDD & 0.114 $\pm$ 0.148 & 0.484 $\pm$ 0.134 & 0.349 $\pm$ 0.174 & 1.669 $\pm$ 0.907 \\
\midrule
DDPP-LB & \textbf{0.436 $\pm$ 0.037} & \textbf{0.897 $\pm$ 0.027} & \textbf{0.806 $\pm$ 0.029} & \textbf{3.703 $\pm$ 0.186} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Shrinking down ribonuclease proteins 9RAT-A and 11BA-A (124 AAs) to 90 AAs while preserving structural fidelity (high TM-Score) and quality (high pLDDT and PTM).}
\setlength{\tabcolsep}{4pt} % Adjust the column spacing
\renewcommand{\arraystretch}{1.2} % Adjust row spacing for better readability
\small % Reduce font size to fit the table within margins
\begin{tabular}{llllll}
\toprule
 & SS-KL & Score & TM-Score & pLDDT & pTM \\
\midrule
Base Model & 3.040 $\pm$ 3.043 & 0.490 $\pm$ 0.116 & 0.245 $\pm$ 0.058 & 0.724 $\pm$ 0.144 & 0.584 $\pm$ 0.226 \\
Best-of-10 & 1.621 $\pm$ 2.804 & 0.690 $\pm$ 0.098 & 0.345 $\pm$ 0.049 & 0.786 $\pm$ 0.023 & 0.737 $\pm$ 0.097 \\
DDPP & 0.640 $\pm$ 1.793 & \textbf{0.722 $\pm$ 0.094} & \textbf{0.361 $\pm$ 0.047} & 0.768 $\pm$ 0.048 & \textbf{0.747 $\pm$ 0.063} \\
RTB & 2.193 $\pm$ 2.724 & 0.581 $\pm$ 0.112 & 0.290 $\pm$ 0.056 & \textbf{0.797 $\pm$ 0.056} & 0.747 $\pm$ 0.093 \\
SVDD & \textbf{3.353 $\pm$ 2.913} & 0.673 $\pm$ 0.083 & 0.337 $\pm$ 0.042 & 0.492 $\pm$ 0.131 & 0.368 $\pm$ 0.171 \\
\bottomrule
\end{tabular}
\end{table}




\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]
    {Plots//proteins/gird_dists_2.png}
    \vspace{-20pt}
    \caption{The distribution of $\beta$-sheet percentage (a), and TM-Score (b) across all methods.}
    \label{fig:dist_metric_2_protein}
\end{figure}
